Levenshtein Training for Word-level Quality Estimation

We propose a novel scheme to use the Levenshtein Transformer to perform the task of word-level quality estimation. A Levenshtein Transformer is a natural fit for this task: trained to perform decoding in an iterative manner, a Levenshtein Transformer can learn to post-edit without explicit supervision. To further minimize the mismatch between the translation task and the word-level QE task, we propose a two-stage transfer learning procedure on both augmented data and human post-editing data. We also propose heuristics to construct reference labels that are compatible with subword-level finetuning and inference. Results on WMT 2020 QE shared task dataset show that our proposed method has superior data efficiency under the data-constrained setting and competitive performance under the unconstrained setting.

==> source/finetuning_old.tex <==
\section{Transfer Learning from Translation to Word-level Quality Estimation}

By training for the translation task, LevT already acquired some initial knowledge of post-editing.
However, there is still some train/inference time mismatch for the word-level QE task regarding (1) the target-side context and (2) the edit tags.
In terms of target-side context, during training, the target-side context is a noised version of the real target sentence in the training set;
during inference, the target-side context is a translation output from an NMT system.
In terms of edit tags, during training, we want the model to predict LCS edit tags that correct the noisy version of the target sentence;
during inference, we want the model to predict TER-style (Levenshtein) edit tags that correspond to human post-editing of NMT outputs.

To address such mismatch, we adopt a two-step transfer learning scheme.
For both stages of transfer learning, we need \emph{translation triplets} (source, MT output, post-edited output) to perform finetuning.
However, in practice, human post-editing resources are quite scarce. 
Hence, like some previous work \cite{lee-2020-two,wang-etal-2020-hw}, we start by performing transfer learning on synthetic translation triplets, followed by real translation triplets constructed with human post-editing.

\noindent\textbf{Synthetic Data Construction}\quad We explore three different methods for translation triplet synthesis:

\begin{itemize}[leftmargin=*,topsep=0pt] \itemsep -2pt
\item \texttt{src-mt-ref}\quad Take a parallel dataset (\texttt{src, ref}) and translate the source sentence with an MT model (\texttt{mt}).
\item \texttt{bt-rt-tgt}\quad Take a target-side monolingual dataset (\texttt{tgt}). Translate the target sentence with an backward MT model (\texttt{bt}) and then translate \texttt{bt} again with an forward MT model, thus creating a round-trip translated output (\texttt{rt}). Use \texttt{rt} as the MT output and the original \texttt{tgt} as the pseudo post-edited output.
\item \texttt{src-mt1-mt2}\quad Take a source-side monolingual dataset (\texttt{src}). Translate the source sentence with a weaker MT model (\texttt{mt1}) and a stronger MT model (\texttt{mt2}). Use \texttt{mt1} as the MT output and \texttt{mt2} as the pseudo post-edited output.
\end{itemize}

\noindent\textbf{Compatibility with Subwords}\quad To the best of our knowledge, previous work on word-level quality estimation either builds models that directly output word-level tags~\cite{lee-2020-two,hu-etal-2020-niutrans-system,moura-etal-2020-ist} or uses simple heuristics to re-assign word-level tags to the first subword token~\cite{wang-etal-2020-hw}.
Since LevT predicts edits on a subword-level starting from translation training, we need to: (1) for inference, convert subword-level tags predicted by the model to word-level tags for evaluation, and (2) for both finetuning stages, build subword-level reference tags.

For inference, the conversion can be easily done by heuristics.
For finetuning, a \emph{naive subword-level tag reference} can be built by running TER alignments on MT and post-edited text after subword tokenization.
However, a preliminary analysis shows that such reference introduces a 10\% error after being converted back to word-level.
Hence, we introduce another heuristic to create \emph{heuristic subword-level tag references}.
The high-level idea is to interpolate the word-level and the naive subword-level references to ensure that the interpolated subword-level tag reference can be perfectly converted back to the word-level references.
Details for the subword tag conversions can be found in Appendix \ref{sec:subword-algos} and Algorithm \ref{algo1} and \ref{algo2} in the appendix.

% \noindent \textbf{Inference}\quad Algorithm \ref{algo1} shows our procedure to convert subword-level tags produced by the model to word-level tags.

% \noindent \textbf{Finetuning}\quad Intuitively, we can build subword-level tag reference by directly using TER alignments built on MT and post-edited text after subword tokenization (BPE, sentencepiece, etc.), which we refer to as naive subword-level reference from now on.
% However, since subword tokenization interacts with the word order error detection (sometimes referred to as ``shifts'') in the TER computation, the naive subword-level references computed this way cannot be perfectly converted back to the word-level references using Algorithm \ref{algo1} introduced above.\footnote{A preliminary analysis shows that the difference is approximately 10\%.}
% Since our model will eventually be evaluated on word-level tags references, finetuning against such naive references is not ideal.

% We propose to build an alternative reference that allows perfect conversion back to their word-level counterparts.
% The high-level idea is to heuristically interpolate the word-level references and the naive subword-level references to ensure the interpolated subword-level tag reference can be perfectly converted back to the word-level references.
% We refer to this interpolated version as \emph{heuristic subword-level reference}.
% The detailed algorithm is shown in Algorithm \ref{algo2}.

% \note{Better name for heuristic subword-level reference?}

